A stabilized mixed formulation for unsteady Brinkman equation based on the method of horizontal lines

In this paper, we present a stabilized mixed formulation for unsteady Brinkman equation. The formulation is systematically derived based on the variational multiscale formalism and the method of horizontal lines. The derivation does not need the assumption that the fine-scale variables do not depend on the time, which is the case with the conventional derivation of multiscale stabilized formulations for transient mixed problems. An expression for the stabilization parameter is obtained in terms of a bubble function, and appropriate bubble functions for various finite elements are also presented. Under the proposed formulation, equal-order interpolation for the velocity and pressure (which is computationally the most convenient) is stable. Representative numerical results are presented to illustrate the performance of the proposed formulation. Spatial and temporal convergence studies are also performed, and the proposed formulation performed well.

==> Sections/S1_UnsteadyBrinkman_Introduction.tex <==
%********************************************;
%  NAME                                      ;
%    S1_UnsteadyBrinkman_Introduction.tex    ;
%********************************************;
\section{INTRODUCTION}
\label{Sec:S1_UnsteadyBrinkman_Introduction}
Among the engineering and environmental issues that demand attention at present, enhanced oil recovery (EOR), carbon-dioxide sequestration, and contaminant transport in heterogeneous media can lay claim to pride of place. The models currently used  are mostly steady state models and reliable computational techniques do exist for them. However, there is a big drawback because it is only if the transient effects are considered that it  will be possible to later study the coupling phenomena that occur due to interaction between different media. Our intention is to propose a stabilized mixed formulation for an unsteady model, since the existing techniques have their own disadvantages. However, before developing the finite element formulation, one needs to turn to theory of mixtures to trace the development of the models.

The foundations of the theory of interacting  continua (also known as theory of mixtures) 
were laid down by Truesdell \cite{Truesdell_Rendiconti_1957_v22_p33,Truesdell_Rendiconti_1957_v22_p158}. One particular physical situation in which it can be gainfully employed  is encountered frequently in the flow of a fluid through a porous solid. Ideally, one would like to be able to predict all quantities of interest in such a situation knowing the nature of the mixture constituents (solid and fluid in this case). But this is easier said than done, for the deformation of the solid due to the flow of fluid through it could be highly non-linear, and the fluid itself may show non-linear behaviour.  Being able to accurately describe such situations quantitatively is the ultimate goal of theory of mixtures and it has been shown in \cite{Rajagopal_Tao} that starting from the balance of linear momentum, one can derive a  whole gamut of mathematical models  pertinent to different situations with varying levels of generality. However, using these models to actually solve realistic engineering problems is another matter altogether. Developing computational techniques to address such models is one of the important thrusts of current research.
%
Herein,  we take into account the transient and viscous effects of the fluid (while still neglecting 
the motion of the solid), which gives rise to \emph{unsteady} Brinkman equation. The main intent 
of the present article is to present a stabilized mixed formulation for the solution of the unsteady 
Brinkman equation.

Darcy's equation \cite{Darcy_1856} describes the flow of a fluid through a porous solid 
due to pressure gradients when a wide variety of  assumptions are justified. It has been 
used to study various phenomena arising in groundwater hydrology 
\cite{Munaf_Lee_Wineman_Rajagopal_M3AS_1993_v3_p231,raats1984applications}, 
enhanced oil recovery \cite{minkoff2003coupled,cusack1992enhanced}, carbon-dioxide 
sequestration \cite{oldenburg2001process,lindeberg1997escape} to name a few. However, 
it should be noted that Darcy's equation is merely an approximation to the balance of 
linear momentum for a fluid as it flows through a rigid porous solid (see References 
\cite{Rajagopal_Tao,Rajagopal_M3AS_2007_v17_p215,Atkin_Craine_QJMAM_1976_v29_p209,
Bowen} for a detailed derivation using the theory of interacting continua, which is 
also known as theory of mixtures). 

Rajagopal \cite{Rajagopal_M3AS_2007_v17_p215} has  shown that, within the context of theory of mixtures, the
Darcy equation can be obtained after making a plethora of assumptions about the solid and the fluid. The assumptions include  neglecting the deformations of the solid, assuming the flow to be steady, assuming a special form for the drag due to the friction at the pores, and many more. The restrictions under which the Darcy equation was derived are rather stringent, and in \cite{Rajagopal_M3AS_2007_v17_p215}, the assumptions  are systematically relaxed and an hierarchy of models is  thus obtained, where the Darcy model is the one derived under the most restrictive assumptions. Moreover, it  has been demonstrated in References
\cite{Kannan_Rajagopal_AMC_2008_v199_p748,Nakshatrala_Rajagopal_arXiv_2009} that for a class of flows involving high pressure gradients, the Darcy equation is a poor approximation. However, despite its drawbacks, it remains the most popular model to describe the flow of fluids through porous solids, and for a large class of flows, it remains applicable. 
In the remainder of the paper, unless otherwise mentioned, the Darcy equation 
tacitly refers to the steady state equation.

If the viscous effects in the fluid are deemed important, as they are in many cases, and  taken into account and  modeled as those of the familiar Navier-Stokes fluid, the eponymous Brinkman model is obtained \cite{brinkman1949calculation}.
By further relaxing the assumption in the Brinkman model  that the flow be steady, we take transient effects into account while still neglecting the inertial non-linearities,  and one thus obtains (as in \cite{Rajagopal_M3AS_2007_v17_p215})
the \emph{unsteady} Brinkman equation, the solution of which is the subject of the present article.

If one desires to use the finite element method to solve the Brinkman equation
(or Darcy equation), then the celebrated Ladyzhenskaya-Babu\v{s}ka-Brezzi (LBB)
condition  \cite{Brezzi_Fortin,Babuska_NumerMath_1971_v16_p322} must be either
satisfied or circumvented. The LBB condition imposes severe restrictions on the
classical mixed formulation with respect to the order of interpolation for the  pressure
and velocity in problems involving incompressibility. In particular, the classical
mixed formulation is unstable for the equal-order interpolation for the velocity and
pressure, which is computationally the most convenient. There is thus a necessity
for stabilized mixed formulations, especially those  that are stable under the
equal-order interpolation for the velocity and pressure. Variational Multiscale
(VMS) formalism provides a systematic way of developing stabilized formulation
\cite{Hughes_CMAME_1995_v127_p387}. Some of the earlier works on mixed methods applied
to flows through porous media are \cite{Burman_Hansbo_JCAM_2007_v198_p35,
Hughes_Masud_Wan_CMAME_2006_v195_p3347,Brezzi_Hughes_Marini_Masud_SIAMJSC_2005_v22_p119,
Arbogast_Wheeler_Yotov_SIAMJNA_1997_v34_p828,Chavent_Cohen_Jaffre_CMAME_1984_v47_p93,
Ewing_Russell_Wheeler_CMAME_1984_v47_p73,Ewing_Heinemann_CMAME_1984_v47_p161}.
%
A thorough discussion of stabilized methods is beyond the scope of this paper,
and a reader interested in  this subject  should refer to
\cite{Burman_Hansbo_NMPDE_2005_v21_p986,Doughlas_Wang_MathComput_1989_v52_p495,
Franca_Hughes_CMAME_1988_v69_p89,Hughes_Franca_Balestra_CMAME_1986_v59_p85,
Hughes_Franca_Balestra_CMAME_1986_v59_p85,Babuska_Oden_Lee_CMAME_1977_v11_p175,
Brooks_Hughes_CMAME_1982_v32_p199,Oden_Jacquotte_CMAME_1984_v43_p231}.

%
\begin{remark}
  While it is possible to avoid a mixed formulation by using primal or single
  field formulations in case of the Darcy equation, such a technique cannot
  be applied to the \emph{unsteady} Brinkman equation. Moreover, the primal
  formulation has the disadvantage of  poor approximation of velocity for low-order finite elements (see \cite{Chen_Huan_Ma, Masud_Hughes_CMAME_2002_v191_p4341}).
\end{remark}
%
This VMS  method for both Brinkman  (or Darcy's equation)  involves decomposing the
velocity field into coarse/resolved scales and fine/unresolved scales. Modeling
of the unresolved scales leads to a multiscale/stabilized form of the corresponding
equation (see Reference \cite{Nakshatrala_Turner_Hjelmstad_Masud_CMAME_2006_v195_p4036}
for details).

The subsequent attempts, quite naturally, were to use the VMS method
to solve the corresponding unsteady problems. The traditional way of
treating the time derivative in the unsteady equation (\emph{unsteady}
Darcy/Stokes/Navier-Stokes) has been to assume that the fine/unresolved
scales are independent of time while allowing the coarse/resolved scales
to depend on both the spatial and temporal variables
\cite{Masud_Khurram_CMAME_2006_v195_p1750,masudcalderer2009variational}.
However, such an assumption is philosophically undesirable as it seems
motivated by the need to somehow solve the fine scale problem rather than
a sound physical basis. For completeness, we have outlined this traditional
way (using a semi-discrete method) of deriving stabilized formulation in
Appendix \ref{Subsec:TransientBrinkman_conventional_derivation}.

Another technique that has been used to treat such unsteady problems is
the so called ``space-time finite elements,'' where the temporal domain is
also discretized via shape functions just like the spatial domain \cite{abedi2006space,palaniappan2004spacetime,bernardigirault}.
However, the disadvantage with this method is that one needs a four-dimensional
mesh for a (spatially) three-dimensional problem, the implementation is not
as convenient, and there are also the same issues with post-processing when
visualizing the numerical results of a (spatially) three-dimensional problem.
%

The method followed in this article sidesteps both the preceding issues discussed
in \cite{Masud_Khurram_CMAME_2006_v195_p1750,masudcalderer2009variational} and
\cite{abedi2006space,palaniappan2004spacetime,bernardigirault}. We use Rothe's method \cite{rothe1930zweidimensionale} (also called the method of horizontal lines) and  avoid the mathematical legerdemain involved in justifying the assumption of the time independence of the fine/unresolved scales.
%

The terminology ``method of lines'' when used with reference to numerical techniques is usually understood to imply method of ``vertical'' lines as distinct from the method of ``horizontal'' lines used in this paper.
The method of lines  \cite{wouwer2001adaptive, schiesser1991numerical} is a favoured numerical technique for the solution of parabolic  partial differential equations (PDEs) wherein the PDE is discretized in all but one dimension and thus reduced to a system of ordinary differential equations (ODEs).
On the other hand, in the method of horizontal lines, the temporal derivative is discretized first (usually by a finite difference scheme) and the original parabolic PDE is thus reduced to a (time-discretized) elliptic PDE.  The entire machinery of techniques and tools used to study elliptic PDEs (which are quite well understood) thus becomes available and therein lies the advantage of the method \cite{ladyzhenskaya1956solution}. In a different context, the method of horizontal lines has been used before. In \cite{deSampaio2005finite} for instance,  a  finite element formulation for transient
incompressible viscous flows stabilized by local time-steps is derived. However, the central idea of the present  paper is different; to use the method of horizontal lines in conjunction with the VMS formalism and derive a consistent  formulation which circumvents an \textit{ad  hoc} assumption that is currently made.


%================================================;
%  Subsection: Main contributions of this paper  ;
%================================================;
\subsection{Main contributions of this paper}
In this paper, we systematically derive a stabilized mixed formulation for
\emph{unsteady} Brinkman equation using the method of horizontal lines and
the variational multiscale formalism. The stabilization terms and parameter
are obtained in a mathematically consistent manner. An important feature is
that the derivation does not need the assumption that the fine-scale variables
do not depend on the time, which is the case with the conventional derivation
of multiscale stabilized formulations for transient mixed problems. Under the
proposed formulation, equal-order interpolation for the velocity and pressure
(which is computationally the most convenient) is stable. We also derive a
stabilized mixed formulation for the \emph{unsteady} Darcy equation as a
special case. We also show through numerical experiments that the proposed 
stabilized formulation posses good spatial and temporal convergence properties. 

%=======================================;
%  Subsection: An outline of the paper  ;
%=======================================;
\subsection{An outline of the paper}
In Section \ref{Sec:S2_UnsteadyBrinkman_Governing_equations}, we outline
the governing equations. In Section \ref{Sec:S3_UnsteadyBrinkman_Stabilized},
we present a stabilized mixed formulation based on the variational multiscale
formalism and the method of horizontal lines for the unsteady Brinkman equation. In Section \ref{Sec:S4_UnsteadyBrinkman_unsteadyDarcy_Stabilized},  the stabilized formulation obtained earlier is specialized for the case of the unsteady Darcy equation. Representative numerical results
are  presented in Section \ref{Sec:S5_UnsteadyBrinkman_Numerical_results}, and
conclusions are drawn in Section \ref{Sec:S6_UnsteadyBrinkman_Conclusions}.

==> Sections/S2_UnsteadyBrinkman_Governing_equations.tex <==
%++++++++++++++++++++++++++++++++++++++++++++++;
%  NAME                                        ;
%    S2_UnsteadyBrinkman_Governing_equations.tex  ;
%++++++++++++++++++++++++++++++++++++++++++++++;
\section{GOVERNING EQUATIONS: UNSTEADY BRINKMAN MODEL}
\label{Sec:S2_UnsteadyBrinkman_Governing_equations}
Let $\Omega \subset \mathbb{R}^{nd}$ be an open bounded domain, where ``$nd$" is
the number of spatial dimensions. Let $\Gamma$ denote the boundary, which is assumed
to be smooth. A position vector is denoted by $\boldsymbol{x} \in \bar{\Omega}$, where
an over-bar denotes the set closure. The time is denoted by $t \in [0, T]$, where $T$ is the
total time of interest. The gradient and divergence operators with respect to $\boldsymbol{x}$
are, respectively, denoted by $\mathrm{grad}[\cdot]$ and $\mathrm{div}[\cdot]$. The velocity
(vector) field is denoted as $\boldsymbol{v}(\boldsymbol{x},t)$, and the pressure (scalar) field
is denoted as $p(\boldsymbol{x},t)$.
%
The coefficient of viscosity, drag, and density are respectively denoted by $\mu$, $\alpha$, and
$\rho$. The prescribed specific body force is  denoted by $\boldsymbol{b}
(\boldsymbol{x},t)$,  while the prescribed velocity on the boundary is denoted by
$\bs{v}^{\mathrm{p}}(\boldsymbol{x},t)$. The unsteady governing equations can
be written as follows:
%-----------------------------;
%  Equation: Stokes equation  ;
%-----------------------------;
\begin{subequations}
  \label{Eqn:UnsteadyBrinkman_governing_equations}
  \begin{align}
    \label{Eqn:UnsteadyBrinkman_linear_momentum}
    & \rho\frac{\partial \boldsymbol{v}}{\partial t} = -\mathrm{grad}[p] - \alpha\boldsymbol{v}
    +\div[\mu \; \grad[\bs{v}]] + \rho \boldsymbol{b} \quad \mathrm{in} \; \Omega \times (0,T) \\
    %
    \label{Eqn:UnsteadyBrinkman_incompressibility_constraint}
    &\mathrm{div}[\boldsymbol{v}] = 0 \quad \mathrm{in} \; \Omega \times (0,T) \\
    %
    %
    \label{Eqn:UnsteadyBrinkman_velocity_BC}
    & \boldsymbol{v}(\boldsymbol{x},t) = \bs{v}^{\mathrm{p}}(\boldsymbol{x},t)
    \quad \mathrm{on} \; \Gamma \times (0,T) \\
    %
    \label{Eqn:UnsteadyBrinkman_IC}
    & \boldsymbol{v}(\boldsymbol{x},0) = \boldsymbol{v}_{0} (\boldsymbol{x}) \quad \mathrm{in} \; \Omega
  \end{align}
\end{subequations}
%
where $\boldsymbol{v}_0(\boldsymbol{x})$ is the prescribed initial velocity. 
Few remarks are in order about the mathematical model given by equations 
\eqref{Eqn:UnsteadyBrinkman_linear_momentum}-\eqref{Eqn:UnsteadyBrinkman_IC}. 

\begin{remark}
The drag coefficient is related to the coefficient of viscosity through 
$\alpha = \dfrac{\mu}{k}$, where $k$ is the coefficient of permeability. 
One obtains unsteady Stokes' equation if the drag term $\alpha \boldsymbol{v}$ 
is neglected. On the other hand, one obtains unsteady Darcy equation if the term 
$\mathrm{div}[\mu \; \mathrm{grad}[\boldsymbol{v}]]$ is neglected and only the 
normal component of the velocity on the boundary is prescribed.

It is noteworthy that a more general form of transient Darcy-Brinkman equation 
can be written as follows: 
  \begin{align}
    \rho\frac{\partial \boldsymbol{v}}{\partial t} = -\mathrm{grad}[p] - \alpha\boldsymbol{v}
    +\div[\mu^{'} \; \grad[\bs{v}]] + \rho \boldsymbol{b}
    \end{align}
    where the factor $\mu^{'}$ can be different from the coefficient of viscosity. 
    %
     Physically, the friction at the pores of the solid as the fluid
flows past it is modeled as  $\alpha(\boldsymbol{v} - \boldsymbol{v}_{\mathrm{solid}})$, 
which reduces to $\alpha\boldsymbol{v}$ under the assumption that the solid is rigid 
and does not undergo any motion.  
On the other hand, the viscous effects within the fluid itself are modeled as 
$\div[\mu^{'} \; \grad[\bs{v}]]$.
    %
    There are adequate discussions in the literature (including the paper by Brinkman 
    \cite{Brinkman_ASR_1947_vA1_p27}) about how the factor $\mu^{'}$ is related to 
    the coefficient of viscosity $\mu$. However, for a medium with high porosity, it is 
    reasonable to assume that $\mu^{'} = \mu$ \cite{Brinkman_ASR_1947_vA1_p27}.
\end{remark}

%------------------------------------------;
%  Remark: Remark about pure velocity BCs  ;
%------------------------------------------;
\begin{remark}
 It is important to note that another constraint must be enforced in order to have a unique solution
  for the pressure. This is usually enforced by demanding that
  \begin{align}
    \int_{\Omega}p \; \mathrm{d} \Omega = 0
  \end{align}
  In numerical simulations, however, it is more convenient to prescribe the pressure at a point,
  which is employed in this paper.
\end{remark}

%--------------------------------------------------------------;
%  Remark: Constitutive equation in terms of D  ;
%--------------------------------------------------------------;
\begin{remark}
The balance of linear momentum for the fluid, on neglecting the non-linear convective term, takes the form
\begin{align}
 \rho\frac{\partial \boldsymbol{v}}{\partial t} =  \div[\boldsymbol{T}] + \rho\boldsymbol{b}
\end{align}
Appealing to frame indifference (or even Galilean invariance),  the partial stress of the fluid  $\boldsymbol{T}$ is actually modeled as
\begin{align}
\boldsymbol{T}= -p\boldsymbol{I} + \mu  \left(\grad[\bs{v}] + \grad[\bs{v}]^T\right)
\end{align}
%
It is only when $\mu$ is a  constant that the incompressibility constraint
$\div[\bs{v}] = 0$ allows the balance of linear momentum to be simplified further and it takes the form as given in
equation \eqref{Eqn:UnsteadyBrinkman_linear_momentum}. This point becomes
crucial in developing (realistic) nonlinear models in which the viscosity depends
on the pressure.
\end{remark}

The main aim of this paper is to develop a stabilized mixed formulation for the
above outlined system of partial differential equations
\eqref{Eqn:UnsteadyBrinkman_linear_momentum}--\eqref{Eqn:UnsteadyBrinkman_IC}.
It is well--known that the semi-discrete formulation based on the classical mixed formulation
has numerical deficiencies. In particular, the equal--order interpolation for the velocity and
pressure (which is computationally the most convenient) is not stable. In the next section
we develop a stabilized mixed formulation for \emph{unsteady} Brinkman equation under
which the equal--order interpolation for velocity and pressure is stable. \emph{An important
aspect is that the derivation does not need the assumption that fine-scale variables do not
depend on the time, which is the case with the conventional derivation of multiscale stabilized
formulations}.

==> Sections/S3_UnsteadyBrinkman_Stabilized_backward_euler.tex <==
%+++++++++++++++++++++++++++++++++++++++++++++++;
%  Section: A new stabilized mixed formulation  ;
%+++++++++++++++++++++++++++++++++++++++++++++++;
\section{A STABILIZED MIXED FORMULATION: UNSTEADY BRINKMAN EQUATION}
\label{Sec:S3_UnsteadyBrinkman_Stabilized}
The proposed formulation is based on the method of horizontal lines (also known
as the Rothe method) \cite{rothe1930zweidimensionale} and variational multiscale
formalism \cite{Hughes_CMAME_1995_v127_p387}. To this end, we shall discretize the
time interval of interest into $N$ instants denoted by $t_n, \;(n = 0, \cdots, N)$.
For simplicity, we shall assume uniform time steps, and shall denote the time step
by $\Delta t := t_n - t_{n-1}$.  However, it should be noted that a straightforward
modification can handle non-uniform time steps. We shall denote the time discretized
version of a given quantity $z(\boldsymbol{x},t)$ at the instant of time $t_n$ as follows:
%--------------------------------------;
%  Equation: Time discretized version  ;
%--------------------------------------;
\begin{align}
  z^{(n)}(\boldsymbol{x}) \approx z(\boldsymbol{x},t_n) \quad n = 0, \cdots, N
\end{align}

In a semi--discrete formulation, the partial differential equation (which depends on
both space and time) is first spatially discretized by (say) the finite element method.
This results in a system of ordinary differential equations (ODEs) or a system of differential
algebraic equations (DAEs), which are numerically integrated using appropriate time stepping schemes.
On the other hand, in the method of horizontal lines (also known as the Rothe's method), the partial
differential equation (which depends on both space and time) is temporally discretized using a time
stepping scheme. This results in another system of partial differential equations, which depends
only on spatial coordinates, and the finite element method or the finite difference method is
typically employed to solve this resulting system of equations. Figure \ref{fig:UnsteadyBrinkman_Rothe}
gives a pictorial description of the method of horizontal lines.

%--------------------------------------;
%  Figure: Method of horizontal lines  ;
%--------------------------------------;
\begin{figure}[htb]
  \centering
\psfrag{u1}{Solve equation \eqref{Eqn:UnsteadyBrinkman_discretized_equations} at time $ t=t_{n+1}$}
\psfrag{u2}{Solve equation \eqref{Eqn:UnsteadyBrinkman_discretized_equations} at time $ t=t_{n}$}
  \includegraphics[scale=0.7]{Figures/UnsteadyBrinkman_horizontal_lines}
  \caption{Rothe's method: The governing equations are solved at each time level
    after discretizing the time interval into discrete time levels.}
  \label{fig:UnsteadyBrinkman_Rothe}
\end{figure}

Herein, we employ the backward Euler time stepping scheme, which is first-order accurate and
unconditionally stable when applied to linear system of ordinary differential equations \cite{Hughes}.
By employing the method of horizontal lines based on the backward Euler scheme to equation
\eqref{Eqn:UnsteadyBrinkman_linear_momentum}~--~\eqref{Eqn:UnsteadyBrinkman_IC}, the
corresponding time discretized equations at time level $t = t_{n+1}$ can be written as follows:
%---------------------------------------------------;
%  Equation: Discretized unsteady Stokes equations  ;
%---------------------------------------------------;
\begin{subequations}
  \label{Eqn:UnsteadyBrinkman_discretized_equations}
  \begin{align}
    \label{Eqn:UnsteadyBrinkman_discretized_LM}
    & \rho\frac{\boldsymbol{v}^{(n+1)} - \boldsymbol{v}^{(n)}}{\Delta t} = -\mathrm{grad}[p^{(n+1)}] -
    \alpha{\boldsymbol{v}^{(n+1)}}  +  \div[\mu\grad[\bs{v}^{(n+1)}]]+ \rho \boldsymbol{b}^{(n+1)} \quad \mathrm{in} \; \Omega \\
    %
    \label{Eqn:UnsteadyBrinkman_discretized_continuity}
    &\mathrm{div}[\boldsymbol{v}^{(n+1)}] = 0 \quad \mathrm{in} \; \Omega \\
    %
    \label{Eqn:UnsteadyBrinkman_discretized_Dirichlet_velocity}
    & \boldsymbol{v}^{(n+1)}(\boldsymbol{x}) =  \bs{v}^{\mathrm{p}}(\boldsymbol{x},t=t_{n+1}) \quad
    \mathrm{on} \; \Gamma \\
    %
    \label{Eqn:UnsteadyBrinkman_discretized_IC}
    & \boldsymbol{v}^{(0)}(\boldsymbol{x}) = \boldsymbol{v}_{0} (\boldsymbol{x}) \quad \mathrm{in} \; \Omega
  \end{align}
\end{subequations}

%----------------------------------------------;
%  Remark: Remark about Brinkman-Stokes equation  ;
%----------------------------------------------;
\begin{remark}
Equation \eqref{Eqn:UnsteadyBrinkman_discretized_LM} can be rearranged to obtain the
following equation:
%----------------------------------------------;
%  Equation: Modified discretized LM equation  ;
%----------------------------------------------;
\begin{align}
  \label{Eqn:UnsteadyBrinkman_discretized_modified_LM}
  \left(\frac{\rho}{\Delta t} + \alpha \right)\boldsymbol{v}^{(n+1)} =
  -\mathrm{grad}[p^{(n+1)}] +   \div[\mu\grad[\bs{v}^{(n+1)}]] + \rho
\left(\boldsymbol{b}^{(n+1)} + \frac{1}{\Delta t}
    \boldsymbol{v}^{(n)}\right) \quad \mathrm{in} \; \Omega
\end{align}
%
At time level $t = t_{n+1}$, the above equation \eqref{Eqn:UnsteadyBrinkman_discretized_modified_LM}
along with equations \eqref{Eqn:UnsteadyBrinkman_discretized_continuity}--\eqref{Eqn:UnsteadyBrinkman_discretized_IC}
resemble the well-known \emph{steady} Brinkman equation with (modified) drag coefficient $\left(\alpha +
\frac{\rho}{\Delta t}\right)$ and (modified) body force  $\left(\boldsymbol{b}^{(n+1)} + \frac{1}{\Delta t}
\boldsymbol{v}^{(n)}\right)$.
\end{remark}

For convenience, let us define $\hat{\alpha}$, $\mathcal{L}(\cdot,\cdot)$,
and $\tilde{\boldsymbol{b}}^{(n+1)}(\boldsymbol{x})$ as follows:
%-----------------------------------------------;
%  Equation: L operator and b_tilde  ;
%-----------------------------------------------;
\begin{subequations}
\begin{align}
%
&\hat{\alpha} := \alpha\Delta t  + \rho \\
%
&\mathcal{L}(\boldsymbol{w},q) := \hat{\alpha} \boldsymbol{w} + \Delta t \;
\mathrm{grad}[q]  - \Delta t  \div[\mu \grad[\bs{w}]]\\
%
&\tilde{\boldsymbol{b}}^{(n+1)} := \Delta t \boldsymbol{b}^{(n+1)} +  \boldsymbol{v}^{(n)}
\end{align}
\end{subequations}
%
Let $L^{2}(\Omega)$ denote the space of square integrable (scalar) functions defined
on $\Omega$. The standard $L^{2}$ inner product over domain $K$ is denoted as
$(\cdot,\cdot)_K$. That is,
%---------------------------------------;
%  Equation: L2 Inner product  ;
%---------------------------------------;
\begin{align}
(a;b)_{K} &\equiv \int_{K} a \cdot b \; \mathrm{d} K \quad \forall a, b \in L^{2}(\Omega)
\end{align}
%
For simplicity, the subscript $K$ will be dropped if the domain is whole of $\Omega$ (that is, $K =
\Omega$). In the remainder of the paper, we shall use the  the following function spaces:
%---------------------------------------;
%  Equation: Function spaces  ;
%---------------------------------------;
\begin{subequations}
\begin{align}
\label{Eqn:MStokes_Function_Space_for_v}
&\mathcal{V}_{t} := \left\{\boldsymbol{v}(\boldsymbol{x}) \; | \; \boldsymbol{v}(\boldsymbol{x}) \in ( H^{1}
(\Omega))^{nd}, \boldsymbol{v}(\boldsymbol{x})
=  \bs{v}^{\mathrm{p}}(\boldsymbol{x},t) \; \mathrm{on} \; \Gamma \right\} \\
%
\label{Eqn:MStokes_Function_Space_for_w}
&\mathcal{W} :=\left\{\boldsymbol{v}(\boldsymbol{x}) \; | \; \boldsymbol{v}(\boldsymbol{x}) \in (H^{1}
(\Omega))^{nd}, \boldsymbol{v}(\boldsymbol{x})
= \boldsymbol{0} \; \mathrm{on} \; \Gamma \right\} \\
%
\label{Eqn:MStokes_Function_Space_for_p}
& \mathcal{P} := \left\{p(\boldsymbol{x}) \in  L^{2}(\Omega) \; | \; \int_{\Omega}p \;
\mathrm{d} \Omega = 0  \right\} \\
%
&\mathcal{Q} := \left\{p(\boldsymbol{x}) \in  H^{1}(\Omega) \; | \; \int_{\Omega}p \;
\mathrm{d} \Omega = 0 \right\}
\end{align}
\end{subequations}
%
where $H^{1}(\Omega)$ is a standard Sobolev space on $\Omega$ \cite{Brezzi_Fortin}. In
the next subsection, we present a derivation of the proposed stabilization mixed formulation.
%
\begin{remark}
 If traction were prescribed on a part of the boundary, then pressure would be uniquely
determined and we need not enforce $\; \int_{\Omega}p \; \mathrm{d} \Omega = 0$.
However, in this paper, we do not consider the possibility of prescribing traction.
\end{remark}

%===========================================;
%  Subsection: A derivation of the proposed stabilized mixed formulation  ;
%===========================================;
\subsection{A derivation of the proposed stabilized mixed formulation}
We start with the classical mixed formulation for equations
\eqref{Eqn:UnsteadyBrinkman_discretized_LM}--\eqref{Eqn:UnsteadyBrinkman_discretized_IC},
which can written as: Find $\boldsymbol{v}^{(n+1)}(\boldsymbol{x}) \in \mathcal{V}_{t = t_{n+1}}$ and
$p^{(n+1)}(\boldsymbol{x}) \in \mathcal{P}$ such that we have
%------------------------------------------------------;
%  Equation: Classical mixed formulation  ;
%------------------------------------------------------;
\begin{align}
\label{Eqn:MStokes_CM_formulation}
& (\boldsymbol{w} ; \hat{\alpha}\boldsymbol{v}^{(n+1)})   + \Delta t (\grad[\bs{w}]; \mu \;
\grad[\bs{v}^{(n+1)}])  - \Delta t (\mathrm{div}[\boldsymbol{w}];p^{(n+1)}) -
\Delta t (q; \mathrm{div}[\boldsymbol{v}^{(n+1)}]) \notag \\
& =  (\boldsymbol{w}; \rho \tilde{\boldsymbol{b}}^{(n+1)})   \quad \forall \boldsymbol{w}(\boldsymbol{x}) \in \mathcal{W}, \; q(\boldsymbol{x}) \in \mathcal{P}
\end{align}
%
As mentioned earlier, the classical mixed formulation has numerical instabilities, and
hence the need for alternate (stabilized) formulations. To this end, let us divide the
domain $\Omega$ into ``$Nele$" non-overlapping subdomains $\Omega^e$ (which,
in the finite element context, will be elements) such that
%-----------------------------------------------------------------;
%  Equation: Dividing Omega into N subdomains  ;
%-----------------------------------------------------------------;
\begin{equation}
  \bar{\Omega} = \overset{Nele}{\underset{e = 1}{\bigcup}} \bar{\Omega}^{e}
\end{equation}
%
The boundary of the element $\Omega^{e}$ is denoted by $\Gamma^{e}:=\bar{\Omega}^{e} -
\Omega^{e}$. We decompose the velocity field $\boldsymbol{v}^{(n+1)}(\boldsymbol{x})$ into
coarse-scale and fine-scale components, indicated as $\boldsymbol{v}^{(n+1)}_{c}(\boldsymbol{x})$
and $\boldsymbol{v}^{(n+1)}_{f}(\boldsymbol{x})$, respectively. That is,
%----------------------------------------------------------------------;
%  Equation: Multiscale decomposition of the velocity  ;
%----------------------------------------------------------------------;
\begin{equation}
  \label{Eqn:MStokes_Decompose_v}
  \boldsymbol{v}^{(n+1)}(\boldsymbol{x}) = \boldsymbol{v}^{(n+1)}_{c} (\boldsymbol{x})
+ \boldsymbol{v}^{(n+1)}_{f}(\boldsymbol{x})
\end{equation}
%
Likewise, we decompose the weighting function $\boldsymbol{w}(\boldsymbol{x})$ into coarse-scale
$\boldsymbol{w}_{c}(\boldsymbol{x})$ and fine-scale $\boldsymbol{w}_{f}(\boldsymbol{x})$ components.
At the outset, we recognize that this multi-scale decomposition can be done irrespective of whether the
problem is linear or non-linear. We further make an assumption that the fine-scale components vanish
along each element boundary. That is,
%------------------------------------------------------------------------;
%  Equation: Fine-scale terms vanish on the boundary  ;
%------------------------------------------------------------------------;
\begin{equation}
  \label{Eqn:MStokes_Fine_Scale_Vanish}
  \boldsymbol{v}^{(n+1)}_{f}(\boldsymbol{x}) = \boldsymbol{w}_{f}(\boldsymbol{x})
= \boldsymbol{0} \quad \mbox{on} \quad \Gamma^{e} \; ; \; e = 1, \cdots, Nele
\end{equation}
%
Let $\mathcal{V}_{c}$ be the function space for the coarse-scale component of the
velocity $\boldsymbol{v}^{(n+1)}_{c}(\boldsymbol{x})$, and $\mathcal{W}_{c}$
be the function space for $\boldsymbol{w}_{c}(\boldsymbol{x})$. The spaces
$\mathcal{V}_{c}$ and  $\mathcal{W}_{c}$ are defined as
%-------------------------------------------------------------------;
%  Equation: Function spaces for v_bar and w_bar  ;
%-------------------------------------------------------------------;
\begin{align}
  \mathcal{V}_{c} := \mathcal{V}_{t}; \; \mathcal{W}_{c} := \mathcal{W}
\end{align}
%
where $\mathcal{V}_{t}$ and $\mathcal{W}$ are as defined earlier in equation
\eqref{Eqn:MStokes_Function_Space_for_v} and equation
\eqref{Eqn:MStokes_Function_Space_for_w}, respectively.
%
Let $\mathcal{V}_{f}$ be the function space for both the fine-scale component of
the velocity $\boldsymbol{v}^{(n+1)}_{f}(\boldsymbol{x})$ and its corresponding
weighting function $\boldsymbol{w}_{f}(\boldsymbol{x})$. It is defined as follows:
%--------------------------------------------------;
%  Equation: Function space U_prime  ;
%--------------------------------------------------;
\begin{align}
  \label{Eqn:MStokes_function_space_for_v_prime}
  \mathcal{V}_{f} := \{\boldsymbol{v}(\boldsymbol{x}) \in \left(H^{1}
(\Omega)\right)^{nd} \; \bigr| \; \boldsymbol{v} (\boldsymbol{x}) =
\boldsymbol{0} \; \mbox{on} \; \Gamma^e; e = 1, \cdots, Nele \}
\end{align}

Substituting equation \eqref{Eqn:MStokes_Decompose_v} into equation
\eqref{Eqn:MStokes_CM_formulation}, one obtains two subproblems.
The coarse-scale and fine-scale subproblems are, respectively, defined as
follows: Find $\boldsymbol{v}^{(n+1)}_{c}(\boldsymbol{x}) \in \mathcal{V}_{c}$,
$\boldsymbol{v}^{(n+1)}_{f}(\boldsymbol{x}) \in \mathcal{V}_{f}$, and
$p^{(n+1)}(\boldsymbol{x}) \in \mathcal{P}$ such that we have
%-----------------------------------------------;
%  Equation: Coarse-scale problem  ;
%-----------------------------------------------;
\begin{subequations}
\begin{align}
\label{Eqn:Brinkman_coarse_scale_problem}
&\left(\boldsymbol{w}_{c}; \hat{\alpha} \boldsymbol{v}^{(n+1)}_{c}\right) + (\boldsymbol{w}_{c}; \hat{\alpha} \boldsymbol{v}^{(n+1)}_{f}) + {\Delta t} \left(\grad[\bs{w}_{c}]; \mu \;\grad[\bs{v}^{(n+1)}_{c}]\right) \notag \\
&+ {\Delta t}(\grad[\bs{w}_{c}]; \mu \; \grad[\bs{v}^{(n+1)}_{f}])
 -{\Delta t} \left(\mathrm{div}[\boldsymbol{w}_{c}];p^{(n+1)}\right)
 - {\Delta t}\left(q;\mathrm{div}[\boldsymbol{v}^{(n+1)}_{c}]\right) \notag \\
&-{\Delta t} (q;\mathrm{div}[\boldsymbol{v}^{(n+1)}_{f}]) = (\boldsymbol{w}_{c};\rho \tilde{\bs{b}}^{(n+1)})
 \quad \forall \boldsymbol{w}_{c}(\boldsymbol{x}) \in \mathcal{W}_{c}, \; q(\boldsymbol{x}) \in \mathcal{P} \\
%
\label{Eqn:Brinkman_fine_scale_problem}
& (\boldsymbol{w}_{f};\hat{\alpha} \boldsymbol{v}^{(n+1)}_{c}) + (\boldsymbol{w}_{f};\hat{\alpha} \boldsymbol{v}^{(n+1)}_{f}) + {\Delta t} \left(\grad[\bs{w}_{f}]; \mu \;\grad[\bs{v}^{(n+1)}_{c}]\right) \notag \\
&+ {\Delta t}(\grad[\bs{w}_{f}]; \mu \; \grad[\bs{v}^{(n+1)}_{f}])
  - {\Delta t}(\mathrm{div}[\boldsymbol{w}_{f}];p^{(n+1)})
  = (\boldsymbol{w}_{f};\rho \tilde{\bs{b}}^{(n+1)})
  \quad \forall \boldsymbol{w}_{f}(\boldsymbol{x}) \in \mathcal{W}_{f}
\end{align}
\end{subequations}
%
The fine scale problem \eqref{Eqn:Brinkman_fine_scale_problem} can be solved (either approximately
or exactly) and substituted into the coarse scale problem \eqref{Eqn:Brinkman_coarse_scale_problem}
to eliminate the fine scale variables completely. But before we attempt to do that, it is necessary to
interpolate the fine-scale variables. [We interpolate the coarse-scale variables using the standard
Lagrangian shape functions.] The fine-scale variables are interpolated using bubble functions. A
bubble function defined over an element is a function that vanishes on the boundary of the element.
The fine-scale variables over an element are interpolated as follows:
%----------------------------------------------------------------;
%  Equation: Interpolation of fine-scale variables  ;
%----------------------------------------------------------------;
\begin{align}
\boldsymbol{v}^{(n+1)}_{f}(\boldsymbol{x}) = b^{e}(\boldsymbol{x}) \boldsymbol{\beta}, \quad
\boldsymbol{w}_{f} (\boldsymbol{x}) = b^{e}(\boldsymbol{x}) \boldsymbol{\gamma}
\end{align}
%
where $b^{e}(\boldsymbol{x})$ is the bubble function while $\boldsymbol{\beta}$ and $\boldsymbol{\gamma}$ are column vectors of size $nd \times 1$. It will be easier to construct a bubble function on the reference element, and use the isoparametric mapping to define it with respect  to the original coordinate system. Therefore, the bubble functions will be functions of  $\boldsymbol{\zeta}$, which is the position vector in isoparametric coordinates. An illustration of all the different bubbles used in this paper is provided in Figure \ref{fig:UnsteadyBrinkman_bubble_functions}.

Solving \eqref{Eqn:Brinkman_fine_scale_problem} for  $\boldsymbol{\beta}$ and substituting
into \eqref{Eqn:Brinkman_coarse_scale_problem}, the proposed stabilized mixed formulation
at time level $t = t_{n+1}$ we arrive at is the following (dropping the suffix $c$ for convenience):
Find $\boldsymbol{v}^{(n+1)}(\boldsymbol{x}) \in \mathcal{V}_{t = t_{n+1}}$ and $p^{(n+1)}
(\boldsymbol{x}) \in \mathcal{Q}$ such that we have
%----------------------------------------------------------------------------------------------;
%  Equation: Proposed stabilized mixed formulation at time level t_n+1  ;
%----------------------------------------------------------------------------------------------;
\begin{align}
\label{Eqn:UnsteadyBrinkman_stabilized_formulation}
& (\boldsymbol{w} ; \hat{\alpha}\boldsymbol{v}^{(n+1)})   + \Delta t (\grad[\bs{w}]; \mu \;
\grad[\bs{v}^{(n+1)}])  - \Delta t (\mathrm{div}[\boldsymbol{w}];p^{(n+1)}) -
\Delta t (q; \mathrm{div}[\boldsymbol{v}^{(n+1)}]) \notag \\
& -  \sum_{e = 1}^{Nele} \left(\mathcal{L}(\boldsymbol{w},q);\tau(\boldsymbol{x})
\mathcal{L}(\boldsymbol{v}^{(n+1)},p^{(n+1)})\right)_{\Omega^e}
=  (\boldsymbol{w}; \rho \tilde{\boldsymbol{b}}^{(n+1)})
 - \sum_{e = 1}^{Nele} \left(\mathcal{L}(\boldsymbol{w},q);\tau(\boldsymbol{x}) \rho
\tilde{\boldsymbol{b}}^{(n+1)} \right)_{\Omega^e}  \notag \\
& \quad \forall \boldsymbol{w}(\boldsymbol{x}) \in \mathcal{W}, \; q(\boldsymbol{x}) \in \mathcal{Q}
\end{align}
%
where the stabilization parameter $\tau(\boldsymbol{x})$ is given by
%-------------------------------------;
%  Equation: Stabilization parameter  ;
%-------------------------------------;
\begin{align}
\tau(\boldsymbol{x}) = b^{e}(\boldsymbol{x}) \left(\int_{\Omega^{e}} b^{e}
(\boldsymbol{x}) \; \mathrm{d} \Omega \right) \left(\int_{\Omega^{e}}
\left(\mu \; \Delta t \; \|\mathrm{grad}[b^{e}]\|^2 + \hat{\alpha} (b^{e})^2 \right)
\; \mathrm{d} \Omega \right)^{-1}
\label{Eqn:UnsteadyBrinkman_stabilization_parameter}
\end{align}
%
where $b^e(\boldsymbol{x})$ is a bubble function. Thus we obtain a formulation which
has additional stabilizing terms compared to classical mixed formulation. A systematic
numerical implementation of the proposed formulation is outlined in Algorithm
\ref{Algo:UnsteadyBrinkman_implementation}. A few remarks about the stabilization
parameter are in order.
%-------------------------------------------------------------;
%  Remark: Remark on tau being well-defined  ;
%-------------------------------------------------------------;
\begin{remark}
We have  $\hat{\alpha}> 0, \;  \mu > 0, \;  \Delta t > 0 $. Also, for $\boldsymbol{x} \in
\Omega^{e},\; (b^{e}(\boldsymbol{x}))^2 > 0, \|\mathrm{grad}[b^{e}]\|^2 > 0 $. The
stabilization parameter $\tau(\boldsymbol{x})$  is thus  well-defined for all permissible
$\hat{\alpha}, \;  \mu$ and $ \Delta t$ since the integrand $\left(\mu \; \Delta t \;
\|\mathrm{grad}[b^{e}]\|^2 + \hat{\alpha} (b^{e})^2 \right) > 0$.
\end{remark}
%------------------------------------------------------;
%  Remark: Remark on bounding the tau  ;
%------------------------------------------------------;
\begin{remark}
On defining
 \begin{align}
  \tau_{\mathrm{avg}} := \dfrac{1}{\mathrm{meas}(\Omega^e)}\int_{\Omega^{e}}
  \tau(\boldsymbol{x}) \; \mathrm{d} \Omega
\end{align}
one can get bounds on $\tau_{\mathrm{avg}}$ for some special cases of interest.
The Poincar\'{e} inequality \cite{Evans_PDE} implies that
\begin{align}
\label{Eqn:UnsteadyBrinkman_Poincare_inequality}
 \int_{\Omega^{e}} (b^{e}(\boldsymbol{x}))^2 \; \mathrm{d} \Omega
 \leq \gamma(\Omega^e)
\int_{\Omega^{e}}\|\mathrm{grad}[b^{e}]\|^2 \; \mathrm{d} \Omega
\end{align}
%
where $\gamma(\Omega^e)$ is a domain-dependent positive constant. Note
that, in the above equation, we have used the fact that the bubble function
vanishes on the boundary. In particular, we have assumed that $b^{e}(\boldsymbol{x})
\in H^{1}_{0}(\Omega^e)$. The elements in a typical finite element mesh will all
be convex domains. For such domains, there are good estimates for the parameter
$\gamma$ (for example, see Reference \cite{bebendorf2003note}).
%
The Cauchy-Schwarz inequality on the other hand  implies
 \begin{align}
\label{Eqn:UnsteadyBrinkman_Cauchy_Schwarz_inequality}
  \left(\int_{\Omega^{e}} b^{e}(\boldsymbol{x}) \; \mathrm{d} \Omega \right)^2
\leq {\mathrm{meas}(\Omega^e)} \left(\int_{\Omega^{e}} (b^{e}(\boldsymbol{x}))^2
\; \mathrm{d} \Omega \right)
 \end{align}
%
The inequalities \eqref{Eqn:UnsteadyBrinkman_Poincare_inequality} and \eqref{Eqn:UnsteadyBrinkman_Cauchy_Schwarz_inequality} immediately yield
\begin{align}
0 < \tau_{\mathrm{avg}} \leq (\hat{\alpha} +\mu\;\Delta t \; \gamma(\Omega^e))^{-1}
\end{align}
%
Specifically, for the unsteady Darcy equation ($\mu = 0$) and the unsteady
Stokes equation ($\hat{\alpha} = \rho$), we have
\begin{subequations}
\begin{align}
& 0 < \tau_{\mathrm{avg}} \leq (\hat{\alpha})^{-1} \quad  \mathrm{if} \; \mu=0 \\
 & 0 < \tau_{\mathrm{avg}} \leq(\rho +\mu\;\Delta t \; \gamma(\Omega^e))^{-1} \quad
\mathrm{if} \;  \hat{\alpha} = \rho
\end{align}
\end{subequations}
%
\end{remark}
%
\begin{remark}
 Readers  consulting the references provided herein  are forewarned of a few errors
and oversights in \cite{Masud_IJNMF_2007_v54_p665} . The boundary
condition prescribed in equation (3) of \cite{Masud_IJNMF_2007_v54_p665}
is appropriate to the Darcy equation and not to the Brinkman equation. A similar comment
applies to equation (4) where the function space for the velocity is defined; such a space is
valid for Darcy equation but not for the Brinkman equation. Moreover, in equation (4), it
ought to read as $\mathrm{trace}(\bs{v}\cdot\bs{n}) = \psi \in H^{-1/2}(\Gamma)$.
%
Finally, the stabilization parameter defined in equation (30) will make sense only if
we understand $\mu\Delta \bs{v}$ to mean $\mu\Delta \bs{v} +\mu\div[ \grad[\bs{v}] ^T ]$.
\end{remark}

%----------------------------------------;
%  Algorithm: Unsteady Brinkman's equation  ;
%----------------------------------------;
\begin{algorithm}[h!]
\caption{Implementation of the proposed formulation}
\label{Algo:UnsteadyBrinkman_implementation}
\begin{algorithmic}[1]
%
\STATE Input: Initial condition $\bs{v}_0$, Time period of integration $T$, time step $\Delta t$
%
\STATE Set $\bs{v}^{(n)}= \bs{v}_{0}$
\STATE Set $t=0$
\WHILE{$t < T$}
%
\STATE $\Delta t = \mathrm{min}(\Delta t, T-t)$,\quad
        $t = t + \Delta t$ \quad
\STATE Using $\bs{v}^{(n)}$,  solve equation \eqref{Eqn:UnsteadyBrinkman_stabilized_formulation}
to obtain $\bs{v}^{(n+1)}, p^{(n+1)}$
\STATE Set $\bs{v}^{(n)} = \bs{v}^{(n+1)}$
%
\ENDWHILE
\end{algorithmic}
\end{algorithm}

%
\begin{remark}
 In the implementation of the algorithm,  all the terms in equation \eqref{Eqn:UnsteadyBrinkman_stabilized_formulation} need not be evaluated repeatedly at each time step since most of them do not depend on the temporal variable.
In fact, only the terms involving $\tilde{\boldsymbol{b}}$ need to be evaluated repeatedly.
\end{remark}

==> Sections/S4_UnsteadyBrinkman_unsteadyDarcy_Stabilized.tex <==
\section{SPECIAL CASE : A STABILIZED MIXED FORMULATION FOR UNSTEADY  DARCY EQUATION}
\label{Sec:S4_UnsteadyBrinkman_unsteadyDarcy_Stabilized}

We now present a stabilized mixed formulation for the unsteady Darcy equation following 
the same procedure as outlined in the previous section. Most of the quantities appearing 
have been defined previously. The ones appearing for the first time are defined here. The 
boundary $\Gamma$ is divided into two parts, denoted by $\Gamma^{v}$ and $\Gamma^{p}$, 
such that $\Gamma^{v} \cap \Gamma^{p} = \emptyset$ and $\Gamma^{v} \cup \Gamma^{p}
=\Gamma$. $\Gamma^{p}$ is the part of the boundary on which the pressure $p$ is prescribed, 
and $\Gamma^{v}$ is that part of the boundary on which the normal component of the velocity 
is prescribed. The prescribed normal component of the velocity on the boundary is denoted by 
$\psi(\boldsymbol{x},t)$, and the prescribed pressure is denoted by $p_0(\boldsymbol{x},t)$. 
The unsteady governing equations can be written as
%-----------------------------;
%  Equation: Stokes equation  ;
%-----------------------------;
\begin{subequations}
  \label{Eqn:UnsteadyDarcy_governing_equations}
  \begin{align}
    \label{Eqn:UnsteadyDarcy_linear_momentum}
    & \rho\frac{\partial \boldsymbol{v}}{\partial t} = -\mathrm{grad}[p] - \alpha\boldsymbol{v}
    + \rho \boldsymbol{b} \quad \mathrm{in} \; \Omega \times (0,T) \\
    %
    \label{Eqn:UnsteadyDarcy_incompressibility_constraint}
    &\mathrm{div}[\boldsymbol{v}] = 0 \quad \mathrm{in} \; \Omega \times (0,T) \\
    %
    \label{Eqn:UnsteadyDarcy_pressure_BC}
    & p(\boldsymbol{x},t) = {p_0}(\boldsymbol{x},t) \quad \mathrm{on} \; \Gamma^{p} \times (0,T) \\
    %
    \label{Eqn:UnsteadyDarcy_velocity_BC}
    & \boldsymbol{v}(\boldsymbol{x},t)\cdot \boldsymbol{n}(\boldsymbol{x}) = \psi(\boldsymbol{x},t)
    \quad \mathrm{on} \; \Gamma^{v} \times (0,T) \\
    %
    \label{Eqn:UnsteadyDarcy_IC}
    & \boldsymbol{v}(\boldsymbol{x},0) = \boldsymbol{v}_{0} (\boldsymbol{x}) \quad \mathrm{in} \; \Omega
  \end{align}
\end{subequations}
%
where $\boldsymbol{n}(\boldsymbol{x})$ is the unit outward normal on the boundary.
%------------------------------------------;
%  Remark: Remark about pure velocity BCs  ;
%------------------------------------------;
\begin{remark}
  It is important to note that if $\Gamma^{v} = \Gamma$, then for a given $\Omega$ (and
  hence given $\Gamma$) $\psi$ cannot be arbitrarily specified. Using the divergence
  theorem it is apparent that $\psi$ must meet the following compatibility condition:
  \begin{align}
    \int_{\Gamma=\Gamma^{v}}{\psi} \; \mathrm{d} \Gamma = 0
  \end{align}
\end{remark}
%
The relevant function spaces for the velocity and pressure fields in case of the 
unsteady Darcy equation are defined as follows:
%---------------------------------------;
%  Equation: Function spaces  ;
%---------------------------------------;
\begin{subequations}
\begin{align}
\label{Eqn:Darcy_Function_Space_for_v}
&\mathcal{\bar{V}}_{t} := \left\{\boldsymbol{v}(\boldsymbol{x}) \; | \; \boldsymbol{v}(\boldsymbol{x}) \in H^{1}
(\mathrm{div};\Omega), \boldsymbol{v}(\boldsymbol{x})\cdot \boldsymbol{n}(\boldsymbol{x})
= \psi(\boldsymbol{x},t) \; \mathrm{on} \; \Gamma^{v} \right\} \\
%
\label{Eqn:Darcy_Function_Space_for_w}
&\mathcal{\bar{W}} :=\left\{\boldsymbol{v}(\boldsymbol{x}) \; | \; \boldsymbol{v}(\boldsymbol{x}) \in H^{1}
(\mathrm{div};\Omega), \boldsymbol{v}(\boldsymbol{x})\cdot \boldsymbol{n}(\boldsymbol{x})
= 0 \; \mathrm{on} \; \Gamma^{v} \right\} \\
%
\label{Eqn:Darcy_Function_Space_for_p}
& \mathcal{\bar{P}} := \left\{p(\boldsymbol{x})  \; | \;  p(\boldsymbol{x}) \in  L^{2}(\Omega)  \right\},
\quad \mathcal{\bar{Q}} := \left\{p(\boldsymbol{x})  \; | \;  p(\boldsymbol{x}) \in  H^{1}(\Omega)  \right\}
\end{align}
\end{subequations}
%
where $H^{1}(\mathrm{div};\Omega)$ is defined by
\begin{align}
 H^{1}(\mathrm{div};\Omega) := \left\{\boldsymbol{v}(\boldsymbol{x}) \in \left(L^{2}
(\Omega)\right)^{nd} \; | \; \mathrm{div}[\boldsymbol{v}] \in L^{2}
(\Omega) \right\}
\end{align}
%

\begin{remark}
 If  we have  $\Gamma^{v} = \Gamma$,  then
 \begin{align}
  & \mathcal{\bar{P}} := \left\{p(\boldsymbol{x}) \in  L^{2}(\Omega) \; | \; \int_{\Omega}p \; \mathrm{d} \Omega = 0  \right\}, \quad
\mathcal{\bar{Q}} := \left\{p(\boldsymbol{x}) \in  H^{1}(\Omega) \; | \; \int_{\Omega}p \; \mathrm{d} \Omega = 0 \right\}
 \end{align}
\end{remark}
%

For convenience, let us define the operator $\mathcal{\bar{L}}(\cdot,\cdot)$, $\hat{\alpha}$
and $\tilde{\boldsymbol{b}}^{(n+1)}(\boldsymbol{x})$ to be
%-----------------------------------------------;
%  Equation: L operator and b_tilde  ;
%-----------------------------------------------;
\begin{subequations}
\begin{align}
&\mathcal{\bar{L}}(\boldsymbol{w},q) := \hat{\alpha} \boldsymbol{w} + \Delta t \; \mathrm{grad}[q]  \\
%
&\hat{\alpha} := \rho + \alpha\Delta t \\
%
&\tilde{\boldsymbol{b}}^{(n+1)} := \Delta t \boldsymbol{b}^{(n+1)} +  \boldsymbol{v}^{(n)}
\end{align}
\end{subequations}
%
A stabilized mixed formulation for unsteady Darcy equation at time level $t = t_{n+1}$ 
can be written as: Find $\boldsymbol{v}^{(n+1)}(\boldsymbol{x}) \in 
\mathcal{\bar{V}}_{t = t_{n+1}}$ and $p^{(n+1)}(\boldsymbol{x}) \in 
\mathcal{\bar{Q}}$ such that we have
%----------------------------------------------------------------------------------------------;
%  Equation: Proposed stabilized mixed formulation at time level t_n+1  ;
%----------------------------------------------------------------------------------------------;
\begin{align}
\label{Eqn:UnsteadyDarcy_stabilized_formulation}
(\boldsymbol{w} ; \hat{\alpha}\boldsymbol{v}^{(n+1)}) & - \Delta t (\mathrm{div}[\boldsymbol{w}];p^{(n+1)}) -
\Delta t (q; \mathrm{div}[\boldsymbol{v}^{(n+1)}]) \notag \\
& - \left(\mathcal{\bar{L}}(\boldsymbol{w},q);\tau(\boldsymbol{x}){\hat{\alpha}}^{-1}
\mathcal{\bar{L}}(\boldsymbol{v}^{(n+1)},p^{(n+1)})\right) \notag \\
&= (\boldsymbol{w}; \rho \tilde{\boldsymbol{b}}^{(n+1)}) - \Delta t (\bs{w}\cdot\bs{n};{p_{0}}^{(n+1)})_{\Gamma^{p}} \notag \\
& - \left(\mathcal{\bar{L}}(\boldsymbol{w},q);\tau(\boldsymbol{x}){\hat{\alpha}}^{-1} \rho
\tilde{\boldsymbol{b}}^{(n+1)} \right) \quad \forall
\boldsymbol{w}(\boldsymbol{x}) \in \mathcal{W}, \; q(\boldsymbol{x}) \in \mathcal{Q}
\end{align}
%
where the stabilization parameter $\tau(\boldsymbol{x})$ is given by
%-------------------------------------;
%  Equation: Stabilization parameter  ;
%-------------------------------------;
\begin{align}
  \tau(\boldsymbol{x}) = b^{e}(\boldsymbol{x}) \left[\int_{\Omega^{e}}
    b^{e}(\boldsymbol{x}) \; \mathrm{d} \Omega \right] \left[\int_{\Omega^{e}}
    (b^{e})^2  \; \mathrm{d} \Omega \right]^{-1}
\end{align}
% 
For simplicity, one can use a constant  representative value of $\tau(\boldsymbol{x}) = 
\tau_{\mathrm{avg}} = \dfrac{1}{2}$ for all elements. A careful discussion on the 
use of the representative value for $\tau_{\mathrm{avg}}$ can be found in References \cite{Nakshatrala_Turner_Hjelmstad_Masud_CMAME_2006_v195_p4036,
Masud_Hughes_CMAME_2002_v191_p4341}).

\begin{remark}
 While this  formulation requires the pressure $p \in H^{1}(\Omega)$, it is possible to use a classical mixed formulation  with different interpolations for the velocity and pressure  so that we only require $p \in L^{2}(\Omega)$. But the relaxation in the requirement comes at the cost of increasing complexity and greater difficulty in implementation. Moreover, the advantage is short-lived because as we proceed in the hierarchy to a Brinkman  model,  we will require further smoothness from the pressure field in any case.
\end{remark}


==> Sections/S5_UnsteadyBrinkman_Numerical_results.tex <==
%+++++++++++++++++++++++++++++++++++++++++++++;
%  Section: Representative numerical results  ;
%+++++++++++++++++++++++++++++++++++++++++++++;
\section{REPRESENTATIVE NUMERICAL RESULTS}
\label{Sec:S5_UnsteadyBrinkman_Numerical_results}
In this section,  we shall show the performance of the proposed stabilized 
formulation using representative numerical examples. We also perform 
spatial and temporal numerical convergence studies. In all the numerical 
simulations, we have employed the equal-order interpolation for the 
velocity and pressure. The drag coefficient, density, and viscosity are 
all taken as $\alpha = \rho = \mu = 1$ for all the cases.

\part{UNSTEADY DARCY EQUATION}
%=======================================;
%  Subsection: One-dimensional problem  ;
%=======================================;
\subsection{One-dimensional problem}
Consider the domain to be of unit length. The body force, boundary conditions,
and initial conditions are, respectively, given by
%--------------------------------;
%  Equation: Problem definition  ;
%--------------------------------;
\begin{subequations}
\label{Eqn: UnsteadyDarcy_case_1D_1}
\begin{align}
b(x,t) &= -\sin(t) + -4x^3\sin(t) + \cos(t) \\
v(0,t) &= v(1,t) = \cos(t)  \\
v(x,0) &= 1
\end{align}
\end{subequations}
%
 For uniqueness, the pressure is prescribed at $x = 0$, and the value is taken to be zero. The analytical
solution is given by
%---------------------------------;
%  Equation: Analytical solution  ;
%---------------------------------;
\begin{subequations}
  \begin{align}
    v(x,t) &= \cos(t) \\
    p(x,t) &=  -x^4\sin(t)
  \end{align}
\end{subequations}
%
The above problem is solved using the proposed formulation, and the computational
domain is divided into $20$ equal-sized two-node linear finite elements. In Figures
\ref{fig:UnsteadyDarcy_case_1_1D_time1} and \ref{fig:UnsteadyDarcy_case_1_1D_time2} the obtained numerical
solution is compared with the exact solution for time instants at $T=1$ and $T=2$,
respectively.

%======================================================;
%  Subsection: Temporal numerical convergence studies  ;
%======================================================;
\subsubsection{Temporal numerical convergence studies}
To study the temporal convergence, we compared the numerical solutions obtained
at time $T= 1$  using successive time steps of magnitude ${10^{-2}}$, $\dfrac{10^{-2}}{2}$,
$\dfrac{10^{-2}}{4}$, $\dfrac{10^{-2}}{8}$ and $ \dfrac{10^{-2}}{16}$ with a  mesh of $128$
elements. The terminal rate of convergence is found to be approximately first order (see
Figure \ref{fig:UnsteadyDarcy_1D_convergence}), which is what is expected of a backward Euler time
discretization scheme.

%=====================================================;
%  Subsection: Spatial numerical convergence studies  ;
%=====================================================;
\subsubsection{Spatial numerical convergence studies}
To study the spatial convergence, we compared the numerical solutions obtained  at
time $T= 1$ using hierarchical meshes (consisting of $8$, $16$, $32$, $64$ and $128$
elements) with a  time step of ${10^{-4}}$. The terminal rates of convergence are
found to be (approximately) first order for the pressure and second order for the
velocity, which are shown Figure \ref{fig:UnsteadyDarcy_1D_convergence}.

%=======================================;
%  Subsection: Two-dimensional problem  ;
%=======================================;
\subsection{Two-dimensional problem}
The computational domain is a bi-unit square. The initial condition for the velocity
is taken to be zero, and homogeneous boundary conditions for the normal component of
the velocity are prescribed on the whole boundary. The test problem is pictorially
defined in Figure \ref{fig:UnsteadyDarcy_2D_problem}. The body force is given by
\begin{subequations}
  \begin{align}
    b_x(x,y,t) &= \left(2\exp(t)-1\right)\sin(2\pi x)\sin(2\pi y) + \sin(\pi t)y(1-y)(1-2x) \\
    b_y(x,y,t) &= \left(2\exp(t)-1\right)\left(\cos(2\pi x)\cos(2\pi y) -
      \cos(2\pi x)\right) + \sin(\pi t)x(1-x)(1-2y)
  \end{align}
\end{subequations}
%
The analytical solution is given by
%----------------------------------------------------------;
%  Equation: Two-dimensional problem: Analytical solution  ;
%----------------------------------------------------------;
\begin{subequations}
  \begin{align}
    v_x(x,y,t) &= \left(\exp(t)-1\right)\sin(2\pi x)\sin(2\pi y), \\
    v_y(x,y,t) &= \left(\exp(t)-1\right)(\cos(2\pi x)\cos(2\pi y)- \cos(2\pi x)) \\
    p(x,y,t)   &= x(1-x)y(1-y)\sin(\pi t)
  \end{align}
\end{subequations}
%
This problem was solved in turn on a T3, Q4 and  an unstructured T3 grid
respectively (see Figure \ref{fig:UnsteadyDarcy_2D_grid}). A grid of size $31\times 31$
was used for the  case of T3 and Q4 elements while $448$ elements were
used in the case of the unstructured T3 grid. A comparison of the exact
and numerical solution at time $T=0.5$ is presented in the contour plots
in Figures \ref{fig:UnsteadyDarcy_2D_problem_solution_T3} --
\ref{fig:UnsteadyDarcy_2D_problem_solution_T3_unstruc}.

%===================================;
%  Subsection: Spatial convergence  ;
%===================================;
\subsubsection{Spatial convergence}
The spatial convergence was studied by comparing numerical solutions obtained
at time $T=0.5$  using successively finer meshes with $5$, $9$, $17$ and $33$
nodes along each side respectively with a time step of magnitude $10^{-3}$.
The terminal rate of convergence is found to be approximately second order
for both pressure and velocity with both four-node quadrilateral and three-node
triangular finite elements (see Figure \ref{fig:UnsteadyDarcy_2D_convergence_spatial}).

\part{UNSTEADY BRINKMAN EQUATION}
%=======================================;
%  Subsection: One-dimensional problem  ;
%=======================================;
\subsection{One-dimensional problem}
Consider the domain to be of unit length. The body force, boundary conditions,
and initial conditions are, respectively, given by
%--------------------------------;
%  Equation: Problem definition  ;
%--------------------------------;
\begin{subequations}
\label{Eqn: UnsteadyBrinkman_case_1D_time1}
\begin{align}
b(x,t) &= \cos(10 \pi t) + 6\pi\exp(t)\cos(6\pi x) -10\pi\sin(10\pi t)\\
v(0,t) &= v(1,t) = \cos(10\pi t)  \\
v(x,0) &= 1
\end{align}
\end{subequations}
%
For uniqueness, the pressure
is prescribed at $x = 0$, and the value is taken to be zero. The analytical
solution is given by
%---------------------------------;
%  Equation: Analytical solution  ;
%---------------------------------;
\begin{subequations}
  \begin{align}
    v(x,t) &= \cos(10\pi t) \\
    p(x,t) &=  \exp(t)\sin(6\pi x)
  \end{align}
\end{subequations}
%
The above problem is solved using the proposed formulation, and the computational
domain is divided into $40$ equal-sized two-node linear finite elements. In Figures
\ref{fig:UnsteadyBrinkman_case_1D_time1} and \ref{fig:UnsteadyBrinkman_case_1D_time2} 
the obtained numericalsolution is compared with the exact solution for time instants at $T=0.1$ 
and $T=0.2$, respectively.

%======================================================;
%  Subsection: Temporal numerical convergence studies  ;
%======================================================;
\subsubsection{Temporal numerical convergence studies}
To study the temporal convergence, we compared the numerical solutions obtained
at time $T= 1$  using successive time steps of magnitude $\dfrac{10^{-2}}{2}$,
$\dfrac{10^{-2}}{4}$, $\dfrac{10^{-2}}{8}$ and $ \dfrac{10^{-2}}{16}$ with a  mesh of $128$
elements. The terminal rate of convergence is found to be approximately first order (see
Figure \ref{fig:UnsteadyBrinkman_1D_convergence}), which is what is expected of a backward Euler time
discretization scheme.

%=====================================================;
%  Subsection: Spatial numerical convergence studies  ;
%=====================================================;
\subsubsection{Spatial numerical convergence studies}
To study the spatial convergence, we compared the numerical solutions obtained  at
time $T= 0.01$ using hierarchical meshes (consisting of $16$, $32$, $64$, $128$ and $256$
elements) with a  time step of ${10^{-5}}$. The terminal rates of convergence are
found to be (approximately) first order for the pressure and second order for the
velocity, which are shown Figure \ref{fig:UnsteadyBrinkman_1D_convergence}.

%=======================================;
%  Subsection: Two-dimensional problem  ;
%=======================================;
\subsection{Two-dimensional problem}
The computational domain is a bi-unit square. The initial condition for the velocity
is taken to be zero, and velocity is  prescribed everywhere on the  boundary. The test problem is pictorially
defined in Figure . The body force is given by
\begin{subequations}
  \begin{align}
    b_x(x,y,t) &= \left(2\exp(t)-1\right)\sin(2\pi x)\sin(2\pi y) + 8\pi^2\left(\exp(t)-1\right)\sin(2\pi x)\sin(2\pi y)  \notag \\
                   & + \pi\exp(t)\cos(\pi x)\sin(\pi y) \\
    b_y(x,y,t) &= \left(2\exp(t)-1\right)\left(\cos(2\pi x)\cos(2\pi y) - \cos(2\pi x)\right)
                        + 8{\pi^2} \left(\exp(t)-1\right)\cos(2\pi x)\cos(2\pi y) \notag \\
                        & -4{\pi^2} \left(\exp(t)-1\right)\cos(2\pi x) +  \pi\exp(t)\cos(\pi y)\sin(\pi x)
  \end{align}
\end{subequations}
%
The analytical solution is given by
%----------------------------------------------------------;
%  Equation: Two-dimensional problem: Analytical solution  ;
%----------------------------------------------------------;
\begin{subequations}
  \begin{align}
    v_x(x,y,t) &= \left(\exp(t)-1\right)\sin(2\pi x)\sin(2\pi y), \\
    v_y(x,y,t) &= \left(\exp(t)-1\right)(\cos(2\pi x)\cos(2\pi y)- \cos(2\pi x)) \\
    p(x,y,t)   &=  \sin(\pi x)\sin(\pi y) \exp(t);
  \end{align}
\end{subequations}
%
This problem was solved in turn on a (six-node triangle element) T6 and (nine-node quadrilateral 
element) Q9 grid respectively (see Figure \ref{fig:UnsteadyBrinkman_bubble_functions}). A grid 
of size $31\times 31$ was used for the  case of Q9 while  a $41\times 41$ grid was used in the 
case of the T6 element. A comparison of the exact and numerical solution at time $T=0.20$ is 
presented in the contour plots in Figures \ref{fig:UnsteadyBrinkman_2D_problem_solution_T6} 
and \ref{fig:UnsteadyBrinkman_2D_problem_solution_Q9}.

\begin{remark}
 The T3 and Q4 elements perform satisfactorily for the unsteady Darcy equation. However in 
 case of the unsteady Brinkman equation, they perform poorly with respect to computation of 
 the pressure, mainly because  the second order term (Laplacian) is identically zero. Hence 
 we have used higher order elements, namely the T6 and Q9 elements for the unsteady 
 Brinkman equation.
%
However, with  higher order elements, the choice of bubble functions is quite critical and is 
by itself an important question. In this case, with better choice of bubbles, the results should 
improve.
\end{remark}

%===================================;
%  Subsection: Spatial convergence  ;
%===================================;
\subsubsection{Spatial convergence}
The spatial convergence was studied at two different time instants, $T=0.01$  and $T=0.1$,  by comparing numerical solutions obtained using successively finer meshes with a constant time step. For the case of
$T=0.01$, we use a time step $\Delta t = 10^{-4}$ while for $T=0.1$, $\Delta t = 10^{-3}$.
In case of the T6 element, meshes consisting of 5, 9, 17 and 33 nodes along each side were used in succession while for the Q9 element, in turn, it consisted of 3, 5, 9, and 17 nodes along each side.
The terminal rate of convergence is found to be approximately second order
for both pressure and velocity with both Q9 and T6 finite elements (see Figure \ref{fig:UnsteadyBrinkman_2D_convergence_spatial_T6} and \ref{fig:UnsteadyBrinkman_2D_convergence_spatial_Q9}).

==> Sections/S6_UnsteadyBrinkman_Conclusions.tex <==
%++++++++++++++++++++++++;
%  Section: Conclusions  ;
%++++++++++++++++++++++++;
\section{CONCLUSIONS}
\label{Sec:S6_UnsteadyBrinkman_Conclusions}
In this paper, we have presented a stabilized mixed formulation for \emph{unsteady} 
Brinkman equation. The proposed formulation is consistently derived based on the 
variational multiscale formalism combined with the method of horizontal lines. The 
derivation does not require the assumption that the fine-scale terms do not depend 
on time, which is required under many of the existing stabilized variational multiscale 
formulations for transient problems. Under the proposed formulation, it has been shown 
numerically that the equal-order interpolation for the velocity and pressure is stable 
(which is not the case with the classical mixed formulation). The performance of the 
proposed formulation is illustrated using various representative numerical examples. 
Spatial and temporal numerical convergence studies are also performed, and the 
proposed formulation performed well.

==> Sections/UnsteadyBrinkman_Figures.tex <==
%===============================================;
%  Figure 12: One-dimensional problem: T = 0.1  ;
%===============================================;
\begin{figure}[p]
  \centering
  \includegraphics[scale=0.8]{Figures/OneD_problem_Brinkman/UnsteadyBrinkman_case_1D_time1}
  \caption{One-dimensional test problem (unsteady Brinkman equation): 
    In this figure the obtained numerical solution is compared with 
    the analytical solution for the time instant at $T = 0.1$. The 
    computational mesh consisted of $40$ equal-sized two-node linear 
    finite elements.}\label{fig:UnsteadyBrinkman_case_1D_time1}
\end{figure}

%===============================================;
%  Figure 13: One-dimensional problem: T = 0.2  ;
%===============================================;
\begin{figure}[p]
  \centering
  \includegraphics[scale=0.8]{Figures/OneD_problem_Brinkman/UnsteadyBrinkman_case_1D_time2}
  \caption{One-dimensional test problem (unsteady Brinkman equation): In this figure the
    obtained numerical solution is compared with the analytical
    solution for the time instant at $T = 0.2$. The computational
    mesh consisted of $40$ equal-sized two-node linear finite
    elements.}\label{fig:UnsteadyBrinkman_case_1D_time2}
\end{figure}

%==========================================================;
% Figure 14: 1D problem: Temporal and spatial convergence  ;
%==========================================================;
\begin{figure}[p]
  \centering
  \subfigure[Temporal convergence using $128$ elements  after  time $T=1$]{
    \includegraphics[scale=0.85]{Figures/OneD_problem_Brinkman/UnsteadyBrinkman_1D_convergence_time}}
  %
  \subfigure[Spatial convergence using $\Delta t = 10^{-5}$  after time $T=0.01$]{
    \includegraphics[scale= 0.85]{Figures/OneD_problem_Brinkman/UnsteadyBrinkman_1D_convergence_space}}
  %
  \caption{One-dimensional test problem (unsteady Brinkman equation): Temporal 
    and spatial convergence. Note that the rate of convergence is in good 
    agreement with the theory.} \label{fig:UnsteadyBrinkman_1D_convergence}
\end{figure}

%==============================;
%  Figure 15: T6 mesh results  ;
%==============================;
\begin{figure}[p]
 \centering
 \subfigure[$p$ (numerical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Brinkman/UnsteadyBrinkmanPre_T6}}
 \subfigure[$p$ (analytical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Brinkman/UnsteadyBrinkmanPre_exact_T6}}
 \subfigure[$v_x$ (numerical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Brinkman/UnsteadyBrinkmanV1_T6}}
 \subfigure[$v_x$ (analytical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Brinkman/UnsteadyBrinkmanV1_exact_T6}}
 \subfigure[$v_y$ (numerical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Brinkman/UnsteadyBrinkmanV2_T6}}
 \subfigure[$v_y$ (analytical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Brinkman/UnsteadyBrinkmanV2_exact_T6}}
 \caption{Two-dimensional test problem (unsteady Brinkman equation) with 
   \emph{six-node triangular finite elements}: Comparison of analytical 
   and numerical solutions at final time $T=0.2$. An equally spaced 
   $41\times41$ grid was used with $\Delta t = 10^{-3}$.} 
 \label{fig:UnsteadyBrinkman_2D_problem_solution_T6}
\end{figure}

%==============================;
%  Figure 16: Q9 mesh results  ;
%==============================;
\begin{figure}[p]
 \centering
 \subfigure[$p$ (numerical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Brinkman/UnsteadyBrinkmanPre_Q9}}
 \subfigure[$p$ (analytical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Brinkman/UnsteadyBrinkmanPre_exact_Q9}}
 \subfigure[$v_x$ (numerical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Brinkman/UnsteadyBrinkmanV1_Q9}}
 \subfigure[$v_x$ (analytical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Brinkman/UnsteadyBrinkmanV1_exact_Q9}}
 \subfigure[$v_y$ (numerical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Brinkman/UnsteadyBrinkmanV2_Q9}}
 \subfigure[$v_y$ (analytical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Brinkman/UnsteadyBrinkmanV2_exact_Q9}}
 \caption{Two-dimensional test problem (unsteady Brinkman equation) with 
   \emph{nine-node quadrilateral finite elements}: Comparison of analytical 
   and numerical solutions at final time $T=0.2$. An equally spaced 
   $31\times31$ grid was used with $\Delta t = 10^{-3}$.} 
 \label{fig:UnsteadyBrinkman_2D_problem_solution_Q9}
\end{figure}

%===========================================================;
%  Figure 17: Two-dimensional problem: Spatial convergence  ;
%===========================================================;
\begin{figure}[p]
 \centering
 \subfigure{
   \includegraphics[scale = 0.85]{Figures/TwoD_problem_Brinkman/UnsteadyBrinkman_2D_convergence_T6_space_smaller_time_step}}
 \subfigure{
   \includegraphics[scale = 0.85]{Figures/TwoD_problem_Brinkman/UnsteadyBrinkman_2D_convergence_T6_space_larger_time_step}}
 \caption{Two-dimensional test problem (unsteady Brinkman equation): The 
   figure presents spatial convergence of the proposed formulation using 
   \emph{six-node triangular finite elements}. The time step and the total 
   time are taken to be $\Delta t = 10^{-4}$ and $T = 0.01$ (top) and 
   $\Delta t = 10^{-3}$ and $T = 0.10$ (bottom), respectively.}
 \label{fig:UnsteadyBrinkman_2D_convergence_spatial_T6}
\end{figure}

%===============================================================================;
%  Figure 18: Two-dimensional problem: Spatial convergence (smaller time step)  ;
%===============================================================================;
\begin{figure}[p]
 \centering
 \subfigure{
   \includegraphics[scale = 0.85]{Figures/TwoD_problem_Brinkman/UnsteadyBrinkman_2D_convergence_Q9_space_smaller_time_step}}
 \subfigure{
   \includegraphics[scale = 0.85]{Figures/TwoD_problem_Brinkman/UnsteadyBrinkman_2D_convergence_Q9_space_larger_time_step}}
 \caption{Two-dimensional test problem (unsteady Brinkman equation): The 
   figure presents spatial convergence of the proposed formulation using 
   \emph{nine-node quadrilateral finite elements}. The time step and the 
   total time are taken to be $\Delta t = 10^{-4}$ and $T = 0.01$ (top) 
   and $\Delta t = 10^{-3}$ and $T = 0.10$ (bottom), respectively .}
 \label{fig:UnsteadyBrinkman_2D_convergence_spatial_Q9}
\end{figure}

==> Sections/UnsteadyDarcy_Figures.tex <==
%==============================;
%  Figure 2: Bubble functions  ;
%==============================;
\begin{figure}[p]
  \centering
  \includegraphics[scale=0.80]{Figures/UnsteadyBrinkman_bubble_functions}
  \caption{This figure shows the bubble functions for various finite elements. The
coordinate axes of the reference/master element are denoted by $\xi_1$ and $\xi_2$.
The locations of the degrees-of-freedom for velocity and pressure nodes in each
element are also indicated.}\label{fig:UnsteadyBrinkman_bubble_functions}
\end{figure}

%============================================;
%  Figure 3: One-dimensional problem: T = 1  ;
%============================================;
\begin{figure}[p]
  \centering
  \includegraphics[scale=0.8]{Figures/OneD_problem_Darcy/UnsteadyDarcy_case_1_1D_time1}
  \caption{One-dimensional test problem (unsteady Darcy equation): In this figure the
    obtained numerical solution is compared with the analytical
    solution for the time instant at $T = 1$. The computational
    mesh consisted of $20$ equal-sized two-node linear finite
    elements.}\label{fig:UnsteadyDarcy_case_1_1D_time1}
\end{figure}

%============================================;
%  Figure 4: One-dimensional problem: T = 2  ;
%============================================;
\begin{figure}[p]
  \centering
  \includegraphics[scale=0.8]{Figures/OneD_problem_Darcy/UnsteadyDarcy_case_1_1D_time2}
  \caption{One-dimensional test problem (unsteady Darcy equation): In this figure the
    obtained numerical solution is compared with the analytical
    solution for the time instant at $T = 2$. The computational
    mesh consisted of $20$ equal-sized two-node linear finite
    elements.} \label{fig:UnsteadyDarcy_case_1_1D_time2}
 \end{figure}

%==========================================================;
%  Figure 5: 1D problem: Temporal and spatial convergence  ;
%==========================================================;
\begin{figure}[p]
  \centering
  \subfigure[Temporal convergence using $128$ elements  after  time $T=1$]{
    \includegraphics[scale=0.85]{Figures/OneD_problem_Darcy/UnsteadyDarcy_1D_convergence_time1}}
  %
  \subfigure[Spatial convergence using $\Delta t = 10^{-4}$  after time $T=1$]{
    \includegraphics[scale= 0.85]{Figures/OneD_problem_Darcy/UnsteadyDarcy_1D_convergence_space1}}
  %
  \caption{One-dimensional test problem (unsteady Darcy equation): Temporal and spatial convergence.
    Note that the rate of convergence is in good agreement with the theory.}
  \label{fig:UnsteadyDarcy_1D_convergence}
\end{figure}

%===================================;
%  Figure 6: 2D problem definition  ;
%===================================;
\begin{figure}[htb]
  \centering
  \includegraphics[scale=0.60]{Figures/TwoD_problem_Darcy/UnsteadyDarcy_2D_case}
  \caption{Two-dimensional problem : A pictorial description of the test problem. The
    computational domain is a bi-unit square. For unsteady Darcy equation: Homogeneous normal components of the
    velocity are prescribed on the whole boundary (that is, $\psi(\boldsymbol{x},t)
    = 0$). The components of the velocity vector are, respectively, denoted by $v_x$
    and $v_y$ so that $v_y = 0$ on $\Gamma_1, \; \Gamma_3$ while  $v_x=0$ on $\Gamma_2, \; \Gamma_4$.
For unsteady Brinkman equation: Velocity is prescribed completely on the boundary, so that, $v_x = v_y = 0$ on $\Gamma_1, \; \Gamma_3$ while $v_x=0,\; v_y =\left(\exp(t)-1\right)(\cos(2\pi y)- 1)$ on $\Gamma_2, \; \Gamma_4$.
To ensure uniqueness of the solution, we enforce pressure to be zero at the  origin O in both cases.}
\label{fig:UnsteadyDarcy_2D_problem}
\end{figure}

%==================================;
%  Figure 7: Computational meshes  ;
%==================================;
\begin{figure}[htbp]
  \centering
  \subfigure[Three-node triangular mesh with $1800$ elements]{
    \includegraphics[scale = 0.35]{Figures/TwoD_problem_Darcy/UnsteadyDarcy_2D_mesh_T3}}
  %
  \subfigure[Four-node quadrilateral mesh with $900$ elements]{
    \includegraphics[scale = 0.35]{Figures/TwoD_problem_Darcy/UnsteadyDarcy_2D_mesh_Q4}}
  %
  \subfigure[Unstructured three-node triangular mesh with $1792$ elements]{
    \includegraphics[scale = 0.35]{Figures/TwoD_problem_Darcy/UnsteadyDarcy_2D_mesh_T3_unstruct}}
  %
  \caption{Two-dimensional test problem: Computational meshes used in the
    numerical simulations.} \label{fig:UnsteadyDarcy_2D_grid}
\end{figure}

%=============================;
%  Figure 8: T3 mesh results  ;
%=============================;
\begin{figure}[p]
  \centering
  \subfigure[$p$ (numerical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Darcy/UnsteadyDarcy_Pre_T3}}
  \subfigure[$p$ (analytical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Darcy/UnsteadyDarcy_Pre_exact_T3}}
  \subfigure[$v_x$ (numerical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Darcy/UnsteadyDarcy_V1_T3}}
  \subfigure[$v_x$ (analytical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Darcy/UnsteadyDarcy_V1_exact_T3}}
  \subfigure[$v_y$ (numerical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Darcy/UnsteadyDarcy_V2_T3}}
  \subfigure[$v_y$ (analytical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Darcy/UnsteadyDarcy_V2_exact_T3}}
  \caption{Two-dimensional test problem (unsteady Darcy equation) with 
    \emph{three-node triangular finite elements}: Comparison of analytical 
    and numerical solutions at final time $T=0.5$. An equally spaced 
    $31\times31$ grid was used with $\Delta t = 10^{-3}$.} 
  \label{fig:UnsteadyDarcy_2D_problem_solution_T3}
\end{figure}

%=============================;
%  Figure 9: Q4 mesh results  ;
%=============================;
 \begin{figure}[p]
   \centering
   \subfigure[$p$ (numerical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Darcy/UnsteadyDarcy_Pre_Q4}}
   \subfigure[$p$ (analytical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Darcy/UnsteadyDarcy_Pre_exact_Q4}}
   \subfigure[$v_x$ (numerical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Darcy/UnsteadyDarcy_V1_Q4}}
  \subfigure[$v_x$ (analytical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Darcy/UnsteadyDarcy_V1_exact_Q4}}
   \subfigure[$v_y$ (numerical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Darcy/UnsteadyDarcy_V2_Q4}}
   \subfigure[$v_y$ (analytical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Darcy/UnsteadyDarcy_V2_exact_Q4}}
   \caption{Two-dimensional test problem (unsteady Darcy equation) with 
     \emph{four-node quadrilateral finite elements}: Comparison of analytical 
     and numerical solutions at final time $T=0.5$. An equally spaced 
     $31\times31$ grid was used with $\Delta t = 10^{-3}$.} 
   \label{fig:UnsteadyDarcy_2D_problem_solution_Q4}
 \end{figure}

%===========================================;
%  Figure 10: T3 unstructured mesh results  ;
%===========================================;
\begin{figure}[p]
  \centering
  \subfigure[$p$ (numerical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Darcy/UnsteadyDarcy_Pre_T3_unstruc}}
   \subfigure[$p$ (analytical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Darcy/UnsteadyDarcy_Pre_exact_T3_unstruc}}
   \subfigure[$v_x$ (numerical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Darcy/UnsteadyDarcy_V1_T3_unstruc}}
  \subfigure[$v_x$ (analytical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Darcy/UnsteadyDarcy_V1_exact_T3_unstruc}}
   \subfigure[$v_y$ (numerical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Darcy/UnsteadyDarcy_V2_T3_unstruc}}
   \subfigure[$v_y$ (analytical)]{\includegraphics[width=0.45\textwidth]{Figures/TwoD_problem_Darcy/UnsteadyDarcy_V2_exact_T3_unstruc}}
  \caption{Two-dimensional test problem (unsteady Darcy equation) with 
    \emph{unstructured grid of three-node finite elements}: Comparison
    of analytical and numerical solutions at final time $T=0.5$. $1792$ 
    elements were used with $\Delta t = 10^{-3}$.} 
  \label{fig:UnsteadyDarcy_2D_problem_solution_T3_unstruc}
\end{figure}

%===========================================================;
%  Figure 11: Two-dimensional problem: Spatial convergence  ;
%===========================================================;
\begin{figure}[p]
  \centering
  \subfigure{
    \includegraphics[scale = 0.85]{Figures/TwoD_problem_Darcy/UnsteadyDarcy_2D_convergence_Q4_space1}}
  \subfigure{
    \includegraphics[scale = 0.85]{Figures/TwoD_problem_Darcy/UnsteadyDarcy_2D_convergence_T3_space1}}
  \caption{ Two-dimensional test problem (unsteady Darcy equation): The figure presents spatial convergence
    of the proposed formulation using four-node quadrilateral elements (top) and
    three-node triangular elements (bottom). The time step is taken to be $\Delta
    t = 10^{-3}$, and the total time is taken to be $T = 0.5$.}
  \label{fig:UnsteadyDarcy_2D_convergence_spatial}
\end{figure}
